Aligned Image-Word Representations Improve Inductive Transfer Across Vision-Language Tasks

An important goal of computer vision is to build systems that learn visual representations over time that can be applied to many tasks. In this paper, we investigate a vision-language embedding as a core representation and show that it leads to better cross-task transfer than standard multi-task learning. In particular, the task of visual recognition is aligned to the task of visual question answering by forcing each to use the same word-region embeddings. We show this leads to greater inductive transfer from recognition to VQA than standard multitask learning. Visual recognition also improves, especially for categories that have relatively few recognition training labels but appear often in the VQA setting. Thus, our paper takes a small step towards creating more general vision systems by showing the benefit of interpretable, flexible, and trainable core representations.

==> full_table_backup.tex <==
\begin{table*}
    \centering 
\setlength\tabcolsep{4 pt}.

    \resizebox{\textwidth}{!}{
    \begin{tabular}{|cccccc||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c||c|c|c||c|}
    \hline
     \rot{answer loss}&
     \rot{\parbox{3cm}{object and \\ attribute losses}}&
     \rot{\parbox{3cm}{separate classifiers \\ and word vectors}}&
     \rot{pretrain classifiers}&
     \rot{relevance features}&
     \rot{binary features}& 
     \rot{\parbox{3cm}{can/could/\\does/do/has}} & 
     \rot{\parbox{3cm}{what does/\\number/name}}& 
     \rot{what brand}&
     \rot{which/who}& 
     \rot{what is/are}& 
     \rot{\textbf{\parbox{3cm}{what is the man/\\woman/person}}}& 
     \rot{\textbf{what color}}& 
     \rot{\textbf{what is in/on}}& 
     \rot{why/how}&
     \rot{how many}&
     \rot{\textbf{\parbox{3cm}{what kind/\\type/animal}}}&
     \rot{what time}& 
     \rot{what room/sport}&
     \rot{where}&
     \rot{none of the above}&
     \rot{is/are/was}&
     \rot{other} &
     \rot{number}&
     \rot{yes/no}&
     \rot{overall accuracy}\\ \hline
     \checkmark & ~                   & ~                   & ~                   & \checkmark & ~                   & 81.8 & 41.9 & 45.9 & 49.0 & 58.3 & 70.5 & 53.5 & 53.6 & 33.8 & 38.4 & 56.8 & 53.9 & 89.8 & 45.8 & 56.0 & 80.2 & 54.5 & 39.2 & 82.1 & 62.9 \\
    \checkmark  & \checkmark & ~                   & ~                   & \checkmark & ~                   & 82.6 & \textbf{46.3} & 48.4 & 51.9 & \textbf{61.3} & 73.2 & 62.7 & \textbf{59.0} & 32.7 & \textbf{39.7} & 59.8 & 57.0 & 90.9 & 47.5 & 58.2 & 81.4 & 58.5 & \textbf{40.8} & 83.1 & 65.5 \\
    \checkmark  & \checkmark & ~                   & ~                   & ~                   & ~                   & \textbf{82.8} & 41.6 & \textbf{52.9} & 52.0 & 61.1 & 74.1 & 62.1 & 57.9 & 33.6 & 39.0 & 60.0 & 51.3 & 91.1 & 48.6 & \textbf{58.5} & 81.4 & 58.8 & 38.8 & 83.0 & 65.3 \\
    \checkmark  & \checkmark & \checkmark & ~                   & ~                   & ~                   & 81.9 & 43.8 & 46.4 & 50.8 & 59.2 & 71.8 & 59.4 & 54.6 & 32.3 & 39.4 & 58.3 & 53.9 & 91.0 & 47.0 & 57.1 & 80.4 & 56.7 & 39.8 & 82.2 & 64.1 \\
    \checkmark  & \checkmark & ~                   & \checkmark & ~                   & ~                   & 80.8 & 43.4 & 44.6 & 48.2 & 60.0 & 72.1 & 59.6 & 56.4 & 32.3 & 39.2 & 58.3 & 56.6 & 89.6 & 47.0 & 55.7 & 79.6 & 56.5 & 40.2 & 81.3 & 63.7 \\
    \checkmark  & \checkmark & ~                   & ~                   & \checkmark & \checkmark & 82.5 & 39.3 & 51.1 & \textbf{52.7} & 61.1 & \textbf{74.9} & \textbf{63.4} & 57.9 & \textbf{34.6} & 39.4 & \textbf{60.7} & \textbf{57.2} & \textbf{91.9} & \textbf{49.8} & 58.3 & \textbf{81.9} & \textbf{59.3} & 38.8 & \textbf{83.4} & \textbf{65.7} \\ \hline
    \end{tabular}}
    \caption{Ablation study of our model to see effects of: (i) joint training (1 vs 2), (ii) using word embeddings in visual classifiers (3 vs 4), (iii) relevance features $\xi$ (2 vs 3), (iv) binary features for \{\textit{yes,no,0,1,2,3}\} (2 vs 6), and (v) pretraining as compared to joint training from scratch (3 vs 5). See Sec \ref{sec:vqa_eval} for details.}
    \label{Tbl:abltionperf}
    \end{table*}

==> teaser_figure.tex <==
\begin{figure}[t]

\centering
\begin{subfigure}[b]{\linewidth}
\includegraphics[width=\linewidth]{images/short_overview.pdf}
\caption{}
\label{fig:short_overview}
\end{subfigure}

\centering
\begin{subfigure}[b]{\linewidth}
\includegraphics[width=\linewidth]{images/yellow_surfboard.pdf}
\caption{}
\label{fig:teaser_interpert}
\end{subfigure}

\caption{(a) We propose a multitask learning model for Vision-Language tasks. Our model projects images and words into a shared representation space. The resulting visual and textual embeddings are then used for each task. We demonstrate the general concept on visual recognition and VQA; (b) We pose VQA in terms of the visual recognition task resulting in a model with interpretable intermediate outputs like region relevance, and object and attribute predictions.}
\end{figure}

==> vqa_word_rarity.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{images/acc_vs_rarity.pdf}
\vspace{-1cm}
\end{center}
  \caption{The effects of jointly training VQA and recognition with and without shared language representations for question types in bold in Table.~\ref{Tbl:abltionperf}. We bin question-answer pairs based on frequency of its least frequent word. We compute each bin's accuracy (primary axis) for each model. We show the percentage reduction in error on the secondary axis. Note that familiarity with $(Q,A)$ words correlates with higher performance. Further, both forms of joint training show larger gains for more frequent question-answers (yellow and green). This is mainly because nouns and adjectives which are more common in VQA also tend to be more common in Visual Genome, resulting in more supervision for the classifiers. Finally, using word embeddings in visual classifiers imposes a structure in the shared representation space that benefits frequent and rare question-answers almost equally (blue).}
\label{fig:acc_vs_rarity}
\end{figure}
